To What Degree Can Language Borders Be Blurred In BERT-based Multilingual Spoken Language Understanding?

This paper addresses the question as to what degree a BERT-based multilingual Spoken Language Understanding (SLU) model can transfer knowledge across languages. Through experiments we will show that, although it works substantially well even on distant language groups, there is still a gap to the ideal multilingual performance. In addition, we propose a novel BERT-based adversarial model architecture to learn language-shared and language-specific representations for multilingual SLU. Our experimental results prove that the proposed model is capable of narrowing the gap to the ideal multilingual performance.

==> COLING 2020 (1) (6)/sections/abstract.tex <==
\begin{abstract}
This paper addresses the question as to what degree a BERT-based multilingual Spoken Language Understanding (SLU) model can transfer knowledge across languages. Through experiments we will show that, although it works substantially well even on distant language groups, there is still a gap to the ideal multilingual performance. In addition, we propose a novel BERT-based adversarial model architecture to learn language-shared and language-specific representations for multilingual SLU. Our experimental results prove that the proposed model is capable of narrowing the gap to the ideal multilingual performance.
\end{abstract}


==> COLING 2020 (1) (6)/sections/acknowledgement.tex <==
\section{Acknowledgement}
Thanks to ...
\label{acknowledgement}


==> COLING 2020 (1) (6)/sections/atis.tex <==
%\section{Results}
\subsubsection{Results}
\begin{table}
\parbox{.5\linewidth}{
\centering
\resizebox{.49\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Exp.}} & \multirow{2}{*}{\textbf{Target}} &  \multirow{2}{*}{\textbf{Model}}& \multicolumn{3}{|c|}{\textbf{Balanced}} & \multicolumn{3}{|c|}{\textbf{Imbalanced}} \\
%\hline
\cline{4-9} 
&&&SemER&SF F1&IC acc.&SemER&SF F1&IC acc.\\
\hline
\hline
\multirow{16}{*}{\rotatebox[origin=c]{90}{\textbf{EN-DE-ES}}}&\multirow{4}{*}{EN} &Naive &  16.06 &90.12& 89.25 & 15.54  & 91.07  & 87.12  \\
& & Ideal & 6.97 & 95.53 & 97.54 & 6.97 & 95.53 & 97.54 \\
& & Multi-lang.& 8.14 & 94.68 & 96.53 & 7.46 & 95.13 & 96.53 \\
& & Lang.-adv.& 8.36 & 94.54 & 96.41 & 7.90  & 94.56 & 97.20 \\
\cline{2-9} 
&\multirow{4}{*}{DE} &Naive & 16.74  & 89.97 & 86.10 & 17.4  & 89.88  & 86.21\\
& & Ideal &8.48  & 94.47 & 95.74 & 8.48  & 94.47 & 95.74 \\
& & Multi-lang.& 9.38 & 93.97  & 95.07 & 10.77 & 93.11 & 94.51 \\
& & Lang.-adv.& 8.51 &94.69  & 95.85 & 10.17& 93.40 & 96.19 \\
\cline{2-9} 
&\multirow{4}{*}{ES} &Naive & 27.17  & 80.26  & 86.10 & 34.38& 74.09& 83.39\\
& & Ideal & 14.45 & 88.37  & 95.82 & 14.45 & 88.37  & 95.82 \\
& & Multi-lang.& 15.79 & 86.94 & 95.33 & 17.24 & 85.91 & 95.94 \\
& & Lang.-adv.& 14.14 & 88.30  & 96.68 & 16.55 & 86.19 & 95.82 \\
\cline{2-9} 
&\multirow{4}{*}{Avg.} &Naive & 19.99  & 86.78 & 87.15 &22.44 & 85.01&85.57 \\
& & Ideal & 9.97 & 92.79 & 96.37 &9.97 & 92.79 & 96.37\\
& & Multi-lang.& 11.10  & 91.86  & 95.64 & 11.82 & \textbf{91.38} & 95.73 \\
& & Lang.-adv.& \textbf{10.34} & \textbf{92.51}  & \textbf{96.31}  & \textbf{11.54 }& \textbf{91.38} & \textbf{96.40} \\
\cline{2-9} 
\hline
\hline

\end{tabular}}
%\caption{Foo}
}
\hfill
\parbox{.5\linewidth}{
\centering
\resizebox{.49\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Exp.}} & \multirow{2}{*}{\textbf{Target}} &  \multirow{2}{*}{\textbf{Method}}& \multicolumn{3}{|c|}{\textbf{Balanced}} & \multicolumn{3}{|c|}{\textbf{Imbalanced}} \\
%\hline
\cline{4-9} 
&&&SemER&SF F1&IC acc.&SemER&SF F1&IC acc.\\
\hline
\hline
\multirow{16}{*}{\rotatebox[origin=c]{90}{\textbf{EN-DE-JA}}}&\multirow{4}{*}{EN} 
&Naive & 17.25 & 89.4  & 86.9 & 10.55 & 92.89 & 95.86 \\
& & Ideal & 6.97 & 95.53 & 97.54 & 6.97 & 95.53 & 97.54  \\
& & Multi-lang. & 8.66 & 94.23  & 96.53  & 9.31 & 93.98  & 95.63\\
& & Lang.-adv.& 7.92 & 94.85 & 95.52 & 7.57  & 94.90  & 94.42\\
\cline{2-9} 
&\multirow{4}{*}{DE} &Naive & 18.32 & 88.84  & 84.87 & 17.4 & 90.10 & 85.43 \\
& & Ideal & 8.48  & 94.47 & 95.74 & 8.48  & 94.47 & 95.74 \\
& & Multi-lang.& 8.70 & 94.44  & 95.63 & 11.21 & 92.91 & 94.28 \\
& & Lang.-adv.& 8.62 & 94.62  & 95.29 & 9.77 & 94.10 & 94.62 \\
\cline{2-9} 
&\multirow{4}{*}{JA} &Naive & 16.54 & 90.70  & 87.36 & 27.1 & 84.4 & 79.91 \\
& & Ideal & 13.15 & 92.40  & 92.21  & 13.15 & 92.40  & 92.21 \\
& & Multi-lang.& 13.98 & 92.01  & 90.07 & 16.16 & 90.6 & 88.6 \\
& & Lang.-adv.& 13.82 & 92.25 & 89.28 & 16.37& 91.19 & 89.61 \\
\cline{2-9} 
&\multirow{4}{*}{Avg.} &Naive & 17.37  & 89.64 & 86.38 & 18.35&89.13 & 87.07 \\
& & Ideal& 9.53  & 94.13  & 95.16 & 9.53  & 94.13  & 95.16\\
& & Multi-lang.&   10.45 & 93.56 & \textbf{94.08} & 12.23 & 92.50& 92.84\\
& & Lang.-adv.& \textbf{10.12} & \textbf{93.91} & 93.36 &  \textbf{11.24} &\textbf{93.40} & \textbf{93.88} \\
\cline{2-9} 
\hline
\hline

\end{tabular}}
%\caption{Bar}
}
\caption{SLU evaluations on trilingual MultiATIS++ (resampled) datasets. Lower numbers indicate better performance for SemER, while higher numbers indicate better performance for slot F1 and intent classification accuracy. Bold numbers indicate better performance between the two multilingual SLU models.}
\label{tbl:atis_tri}
\end{table}

\begin{table}
\parbox{.5\linewidth}{
\centering
\resizebox{.49\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Exp.}} & \multirow{2}{*}{\textbf{Target}} &  \multirow{2}{*}{\textbf{Model}}& \multicolumn{3}{|c|}{\textbf{Balanced}} & \multicolumn{3}{|c|}{\textbf{Imbalanced}} \\
%\hline
\cline{4-9} 
&&&SemER&SF F1&IC acc.&SemER&SF F1&IC acc.\\
\hline
\hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{EN-DE}}}&\multirow{4}{*}{EN} &Naive & 9.12 & 94.12     & 95.63 & 8.22  & 94.68  & 96.98  \\
& & Ideal & 6.97 & 95.53 & 97.54 & 6.97 & 95.53 & 97.54 \\
& & Multi-lang.& 9.34& 94.06 & 94.74   & 7.24 & 95.36  & 97.31    \\
& & Lang.-adv.& 7.82 & 94.77   & 95.74 & 7.08 & 95.21  & 97.42  \\
\cline{2-9} 
&\multirow{4}{*}{DE} &Naive& 14.65 & 91.23   & 88.12 & 15.35 & 90.88  & 87.56  \\ 
& & Ideal &8.48  & 94.47 & 95.74 & 8.48  & 94.47 & 95.74 \\
& & Multi-lang.&  9.57& 93.98   & 94.96 &  8.26 & 94.17  & 96.08  \\
& & Lang.-adv.& 9.11 & 94.16   & 95.63 & 9.55  & 93.83  & 95.52   \\

\cline{2-9} 
&\multirow{4}{*}{Avg.} &Naive&  11.89 & 92.68  & 91.88 &  11.79 & 92.78  & 92.27 \\
& & Ideal & 7.73 & 95.00 & 96.64 &  7.73 & 95.00 & 96.64 \\
& & Multi-lang.& 9.46  & 93.98  & 94.85 & 8.36 & \textbf{94.77}  & 96.17  \\
& & Lang.-adv.& \textbf{8.47} &  \textbf{94.47} & \textbf{95.69} & \textbf{8.32} & 94.52  & \textbf{96.47}  \\
\cline{2-9} 
\hline
\hline

\end{tabular}}
%\caption{Foo}
}
\hfill
\parbox{.5\linewidth}{
\centering
\resizebox{.49\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Exp.}} & \multirow{2}{*}{\textbf{Target}} &  \multirow{2}{*}{\textbf{Method}}& \multicolumn{3}{|c|}{\textbf{Balanced}} & \multicolumn{3}{|c|}{\textbf{Imbalanced}} \\
%\hline
\cline{4-9} 
&&&SemER&SF F1&IC acc.&SemER&SF F1&IC acc.\\
\hline
\hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{EN-JA}}}&\multirow{4}{*}{EN} 
&Naive & 10.29 & 93.03  & 95.97 & 8.96 & 94.19  & 94.62  \\
& & Ideal & 6.97 & 95.53 & 97.54 & 6.97 & 95.53 & 97.54  \\
& & Multi-lang. & 8.87 & 94.01   & 96.97   & 8.82 & 94.39   & 95.63\\
& & Lang.-adv.& 8.55 & 94.28  & 95.86  & 7.54  & 95.11   & 96.86 \\
\cline{2-9} 
&\multirow{4}{*}{JA} &Naive & 18.13 & 89.71   & 85.21 & 20.77  & 87.94  & 84.09  \\
& & Ideal & 13.15 & 92.40  & 92.21  & 13.15 & 92.40  & 92.21 \\
& & Multi-lang. & 13.87 &  92.35  & 89.28   & 15.44& 91.71   & 86.34\\
& & Lang.-adv.& 13.21 & 92.81  & 89.05  & 14.37  & 92.41   & 87.70 \\
\cline{2-9} 
&\multirow{4}{*}{Avg.} &Naive &14.21  & 91.37  & 90.59 & 15.32  & 91.07  & 89.36 \\
& & Ideal& 10.06 &  93.97 &94.88 &10.06 &  93.97 &94.88  \\
& & Multi-lang. & 11.37& 93.18  & \textbf{93.13}   & 12.13 & 93.05   & 90.99\\
& & Lang.-adv.& \textbf{10.88} & \textbf{93.55} & 92.46  & \textbf{10.96}  & \textbf{93.76 }  & \textbf{92.28} \\
\cline{2-9} 

\hline
\hline

\end{tabular}}
%\caption{Bar}
}
\caption{SLU evaluations on bilingual MultiATIS++ (resampled) datasets. Lower numbers indicate better performance for SemER, while higher numbers indicate better performance for slot F1 and intent classification accuracy. Bold numbers indicate better performance between the two multilingual SLU models.}
\label{tbl:atis_bi}
\end{table}
\begin{figure}[ht]
    \parbox{0.5\linewidth}{
        \centering
        \resizebox{0.5\textwidth}{!}{
            \centering
            \includegraphics[width=9cm]{figs/semer-tri-grey-small.png}
        }
    }
    \parbox{0.5\linewidth}{
        \centering
        \resizebox{0.5\textwidth}{!}{
            \centering
            \includegraphics[width=9cm]{figs/semer-bi-grey-small.png}
        }
    }
    \caption{Average semantic error rate (SemER) comparisons on MultiATIS++ (resampled).}
    \label{fig:semer_compare}
\end{figure}


Table \ref{tbl:atis_bi} and Table \ref{tbl:atis_tri} show our experimental results on bilingual and trilingual datasets, respectively. As can be seen, both of the two multilingual SLU models consistently outperform the Naive baseline, meaning that multilingual techniques can effectively transfer knowledge across different languages. The relative improvements in avg. SemER range from 19.98\% on Balanced (EN-JA) to  48.58\% on Imbalanced (EN-DE-ES) scenarios. Interestingly, this holds even on the groups of (EN, JA) and (EN, DE, JA) in which JA is linguistically distant to the other languages. Moreover, the multilingual models surpass Naive performance not only on the average performance over the target languages but also on every individual language. 

Overall, there is still a gap between the Ideal performance and the two multilingual SLU models. The largest difference in avg. SemER is observed on Imbalanced(EN-DE-JA) where Multi-lang. is 28.33\% relatively worse than Ideal. However, the fact that the absolute gap of 2.7\% here is rather small compared to the absolute improvement of 6.12\%  over Naive baseline, confirms the effectiveness of the multilingual techniques. 

%However, the fact that the absolute gap of 2.7\% here is rather small while the absolute improvement of 6.12\% absolute compared to the Naive baseline confirms the effectiveness of the multilingual techniques. 

The experimental results also prove our hypothesis that using both language-shared and language-specific features can narrow the gap to the Ideal performance. In particular, Lang.-adv. gives lower average semantic error rates (SemER) than Multi-lang. in all of our scenarios. The other two metrics, SF F1 and IC acc., are also improved by Lang.-adv. over  Multi-lang. in 5 out of 6 datasets. Surprisingly,  Lang.-adv. even exceeds or comes very close to the Ideal performance for ES and DE on the dataset Balanced (EN-DE-ES), and for DE on the dataset Balanced (EN, DE, JA). In addition, the results show that there is a significant difference in model performance on the balanced and imbalanced versions of the datasets. Across the different trilingual and bilingual settings, the imbalanced versions of the dataset have on average a lower performance than their balanced counterparts. This shows that while transferring knowledge across different languages works, there is still a drop in performance if data available for one of the languages is scarce.

Another interesting finding can be seen in the comparison of the two bilingual settings, as the language pair EN-DE consistently performs better than EN-JA. This is to be expected as JA is more distant to EN than EN is to DE as EN and DE are both Germanic languages.

Fig. \ref{fig:semer_compare} visualizes the comparisons of the two multilingual SLU models against the Naive and Ideal performance. 

\subsubsection{Comparison to state-of-the-art and model complexity}
Using the same training, development and testing data as \newcite{multiatis++}, our monolingual SLU model obtains 97.54 intent accuracy and 95.53 slot F1 on English ATIS (Ideal baseline on English). These results are comparable to the BERT-based performances reported by \newcite{multiatis++}, which are 97.20 intent accuracy and 95.57 slot F1. This confirms the strength of our baselines. 
%Comparison with SOTA On English ATIS, \cite{chen19} report 97.5% intent accuracy and
%96.1% slot F1 when using BERT with their proposed stack-propagation architecture. This is comparable to our target only with BERT scores in
%Table 2.

A common concern with a BERT-based model is about its complexity. In fact, using CNN encoders prevents our adversarial model Lang.-adv. from a dramatic increase in the number of parameters. On the trilingual datasets, the number of parameters is about 190.4M which is just 5.6\% more than that of Multi-lang. We also found that replacing CNN encoders by BERT encoders not only increases the number of model parameters to 260.9M but also does not bring significant gain in model performance. 

==> COLING 2020 (1) (6)/sections/conclusion.tex <==
\section{Conclusion}
We have addressed the question of to what degree language borders can be blurred in BERT-based multilingual SLU. Our experimental results on a wide range of multilingual SLU datasets showed that although mBERT is substantially good in blurring language borders even on distant language groups, there is still a gap to the ideal multilingual performance. To narrow this gap, we proposed an adversarial model architecture which uses BERT and CNN encoders to learn language-shared and language-specific representations for SLU. 

\label{conclusion}


==> COLING 2020 (1) (6)/sections/data.tex <==
% !TEX root = ../multilingual_DNN_coling.tex

\section{Datasets}
We evaluate our model on a resampled version of the publicly available MultiATIS++ dataset \cite{multiatis++}, which contains parallel SLU data from several languages, and thus allows evaluating performance in relation to the ideal and naive baselines. In addition, we evaluate our model on real-world SLU data to explore the impact of our proposed adversarial model architecture in a real-world scenario.
\subsection{Publicly available data}
The ATIS (``Air Travel Information Service") dataset \cite{atis} is one of the most well-known datasets for evaluating SLU models. It was created by having participants solve given air travel planning scenarios, and then the resulting queries were manually transcribed and annotated. MultiATIS \cite{multiatis} extended the original dataset by adding two additional languages (Turkish and Hindi), and recently six further languages (Spanish, German, Chinese, Japanese, Portuguese, French) were added yielding MultiATIS++ \cite{multiatis++}. For our experiments, we focus on four languages for which we have both real-world and MultiATIS++ data available, i.e. English (EN), German (DE), Spanish (ES) and Japanese (JA).

In MultiATIS++, the data for additional languages were created by manually translating the original English utterances. For translations, several of the slot values, such as city names, were simply kept, yielding e.g. German requests about American airports. We consider keeping a large numbers of slot values the same across languages as being unrealistic, as in real-world applications typically slot value usage differs across locales. In addition, this makes it unrealistically easy for evaluating multilingual models, which may show strong performance just by remembering slot values from the source language.    
%The extension contains six new languages, namely Spanish, German, Chinese, Japanese, Portuguese.
%, and French, which brings the overall corpus to nine different languages from four language families. 
%we want to make a direct comparison between the ATIS data and the real-world data set. Therefore we limit the ATIS data to only four of the nine available languages (\emph{English}, \emph{German}, \emph{Spanish},  \emph{Japanese}). 
%Additionally, one of the characteristics of the MultiATIS++ dataset \cite{multiatis++} is the fully parallel data between all languages. In the real-world such a dataset is difficult and cost intensive to obtain, which makes the evaluation results obtained by evaluating on parallel data less significant for production use cases. 
To make the data more realistic we resampled slot values for the city name slot, which is the most frequent one in the data. In particular, we replaced slot values for the city name slot using the cities with the biggest airports in the region, i.e. the top 30 European airport cities for DE, the top 24 Latin-American airport cities for ES and the top 28 Japanese airport cities for JA.

Across the four languages considered for our experiments, MultiATIS++ (resampled) comprises 4488, 490 and 893 utterances for train, dev and test respectively. The data cover 18 intents and 84 slots. %We are considering to make the resampled dataset available upon the acceptance of this paper.

%created a non-parallel dataset by resampling the MultiATIS++ data on the city name slot. The slot was used as it has the highest occurence of all the available slots and by choosing cities from non-overlapping regions of the world it makes the data non-parallel. As the original data from MultiATIS++ already uses American city names and it is only necessary to resample three of the four languages to create a non-parallel dataset, we decided to use the English data as is. This is also shown in the table \ref{tab:dataset-statistics}, where the English numbers for both datasets are the same. The other languages were resampled on the city name slot using the cities with the biggest airports in the region: the top 30 european airport cities for German, the top 24 latin-american airport cities for Spanish and the top 28 japanese airport cities for Japanese. 

%\begin{table}[h]
%	\begin{center}
%		\begin{tabular}{l|l|rrr|rrr|cc}
%			Dataset & Language & %\multicolumn{3}{c|}{Utterances} & %\multicolumn{3}{c|}{Tokens} & %\multicolumn{1}{l}{Intents} & \multicolumn{1}{l}{Slots} %\\
%			&  & \multicolumn{1}{c}{train} & %\multicolumn{1}{c}{dev} & \multicolumn{1}{c|}{test} & %\multicolumn{1}{c}{train} & \multicolumn{1}{c}{dev} & %\multicolumn{1}{c|}{test} & \multicolumn{1}{l}{} & %\multicolumn{1}{l}{} \\ \hline
%			\multirow{4}{*}{MultiATIS++} & English & 4488 %& 490 & 893 & 50755 & 5445 & 9164 & 18 & 84 \\
%			& German & 4488 & 490 & 893 & 51518 & 5552 & 9577 & 18 & 84 \\
%			& Spanish & 4488 & 490 & 893 & 55683 & 5985 & %10338 & 18 & 84 \\
%%			& Japanese & 4488 & 490 & 893 & 135109 & %14542 & 26235 & 18 & 84 \\ \hline
%			\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Mu%ltiATIS++\\ resampled\end{tabular}} & English & 4488 & %490 & 893 & 50755 & 5445 & 9164 & 18 & 84 \\
%			& German & 4488 & 490 & 893 & 50861 & 5493 & %9270 & 18 & 84 \\
%			& Spanish & 4488 & 490 & 893 & 59199 & 6314 & %10774 & 18 & 84 \\
%			& Japanese & 4488 & 490 & 893 & 107361 & %11576 & 20777 & 18 & 84
%		\end{tabular}
%	\end{center}
%	\caption{Comparison of the data statistics for the %MultiATIS++ corpus and the resampled version. Utterance and token numbers (characters for Japanese) are given for each of the four languages and are split by training (train), development (dev), and test set. In addition, the number of intents and slots (before adding the BIO tags) are provided.}
%	\label{tab:dataset-statistics}
%\end{table}
%In table \ref{tab:dataset-statistics} a comparison of the data statistics of the resampled dataset and the original version is shown. It shows that in both versions of the data the number of utterances are the same for training, development and testing set as well as the distribution of utterances between them. This is due to the fact that the existing utterances were used without any down- or upsampling. Instead, the token statistics show some changes for German, Spanish, and Japanese. This is due to using different city names, which have a different amount of tokens. One example would be the German city "\emph{Frankfurt am Main}" vs "\emph{Philadelphia}" in the original English data. For English the number of tokens doesn't change as we used the original data in both datasets. Intents and slots do not change between the two versions.
\paragraph{Balanced and Imbalanced multilingual datasets} We created two variants of the resampled data to allow detailed evaluation of our proposed approach in relation to different \textit{multilingual} SLU scenarios, i.e. a balanced and an imbalanced variant. The imbalanced version reflects a real-world scenario, where usually an application is rolled out to different locales over time, yielding different data amounts, with the English version usually being the first and having highest data amounts. %Note that, we adjusted only the train and dev parts, and kept the test parts the same.
%one is balanced and one is imbalanced to show the effects of having languages with smaller amounts of available data. This imbalanced scenario is also more aligned with the data we have in the real-world, where a lot of the data is available in English but not so much for other languages. 

To create trilingual balanced versions, for each train and dev, we split the utterance ids\footnote{Each utterance id refers to four translated utterances in EN, DE, ES and JA.} into three equal parts, and we construct mixed datasets by taking disjoint subsets across languages. To create imbalanced versions, the train and dev data were split into three parts across languages: 50\%, 33\%, and 17\%. The largest subset corresponds to EN data, the second largest to DE data, and the smallest part is either ES or JA data for the two sets of three languages respectively. The goal was to select the data in a way that with multilingual data we have all the available utterances but in three languages. The split for the balanced versions was 50/50, and for the imbalanced version it was 70/30, with 70\% for EN and 30\% for DE or JA.

Each of the target languages has a test set taken from MultiATIS++ (resampled).
\subsection{Real-world data}
We created a dataset comprising real-world data by extracting random samples from a commercial large-scale SLU system. The data are representative of user requests to voice-controlled devices, and they were manually annotated with slot and intent labels. Aiming to get a diverse dataset, we included data from three domains\footnote{In real-world SLU applications usually the intents are split into different domains; the data in our experiments are still all from the same overall source.} (\emph{Music}, \emph{Books}, \emph{Video}). To reflect the real-world use case, where user frequency and hence data size differs across domains, we extracted samples of different sizes. In particular, we use 20k, 10k and 5k user utterances for \emph{Music}, \emph{Video} and \emph{Books}, respectively, yielding a total of 35k utterances for each language. Each domain sample was split into 80\% training, 10\% dev and 10\% test data. Note that unlike the MultiATIS++ data, the real-world data are not parallel, as they were not artificially ported from one language to another. 

\label{data}


==> COLING 2020 (1) (6)/sections/experiments.tex <==
% !TEX root = ../multilingual_DNN_coling.tex
\section{Experiments}
In this section, we first describe the multilingual performance evaluation and experimental settings. Afterwards, we present experiments on the resampled MultiATIS++ dataset and subsequently experiments with real-world-data. 
\subsection{Multilingual performance evaluation}
To address the question of to what degree language borders can be blurred in BERT-based multilingual SLU, we compare two multilingual SLU models as discussed in Sec. \ref{lbl:method} with the Ideal and Naive baselines on the Balanced and Imbalanced multilingual datasets (see Sec. \ref{data}). We denote the standard and adversarial multilingual SLU models as Multi-lang. and Lang.-adv., respectively. 
The Ideal and Naive baselines on each of the target languages are computed as in Sec. \ref{lbl:ideal-flawed} by using the BERT-based model described in Sec. \ref{slu-bert} as the monolingual model $\mathcal{M'}$.
%For each scenario of balanced (EN-DE-ES), imbalanced (EN-DE-ES), balanced (EN-DE-JA), imbalanced (EN-DE-JA), balanced (EN-DE), imbalanced (EN-DE), balanced (EN-JA), and imbalanced (EN-JA), we compute the performance of the two SLU models and the ``Ideal" and ``Flawed" on each of the target language using the test sets in MultiATIS++ resampled.

%\begin{itemize}
%\setlength{\parskip}{-3pt}
%    \item Flawed: The performance of ``Flawed" on language $l$ is computed as the performance of a monolingual model trained on $d^l$ on the $l$ version of the test set in $\bf D$.
%    \item Ideal: A monolingual model trained on ${\bf D}^l$ where $l$ is a language in the dataset.
%    \item Multi-lang.: A standard multilingual SLU model trained on $\bf D$.
%    \item Lang.-adv.: Our proposed adversarial and multilingual SLU model trained on $\bf D$.
%\end{itemize}
%The definitions of $d^l$ and ${\bf D}^l$ can be found in Section \ref{lbl:ideal-flawed}.
%In addition, to further evaluate the performance of our proposed adversarial SLU model, we evaluate the two multingual SLU models on the real-world SLU dataset.

\subsubsection{Settings} In all of our experiments, we use pre-trained multilingual BERT \cite{mBERT}. Notably, we compared pre-trained multilingual BERT and monolingual BERT in monolingual models, and found that they have similar performance on our datasets. The IC and SF decoders each have two dense layers of size 768 with gelu activation.  The dropout values used in IC and SF decoders are 0.5 and 0.2, respectively. The language decoders each have 1 dense layer of size 768 with gelu activation, and dropout value of 0.5. The CNN encoders each have one 2D convolutional layer with kernel size and hidden dim set to 3 and 512, respectively. All encoders use max-pooling for computing sentence representations.  For optimization, we use Adam optimizer with learning rate 0.1 and a Noam learning rate scheduler, and we trained our models with mini-batch size of 32 on a single GPU. For adversarial models, the $\alpha_d, \alpha_i, \alpha_s, \alpha_p, \beta_d$ hyper-parameters are set to (1.0, 1.0, 1.0, 1.0, 0.2) and (1.0, 1.0, 0.5, 0.5, 0.2) in our trilingual and bilingual experiments, respectively. The models are trained for 180 epochs with early stopping. We choose the best epoch based on the validation score of Task 2 in Alg. \ref{alg:adv}. 

To evaluate our models, we use the standard SLU metrics,  i.e.  F1 for slot filling (computed using the CoNLL2002 script) and accuracy for intent classification. In addition, following 
\newcite{gaspers2018} we use a semantic error rate, which measures IC and SF jointly and is defined as follows:
\begin{equation}
\textrm{\emph{SemER}} = \frac{\#(\textrm{slot+intent errors})}{\#\textrm{slots in reference + 1}}\end{equation}
\label{experiments}
\input{sections/atis}

==> COLING 2020 (1) (6)/sections/intro.tex <==
% !TEX root = ../multilingual_DNN_coling.tex

\section{Introduction}
Recently, modern voice-controlled devices with virtual assistants like Alexa, Siri, and Google Assistant, have been working their way into every activity of our daily life from playing a song to driving a car. 
Spoken Language Understanding (SLU) models interpreting the semantic meaning conveyed by an user's spoken utterance, are the AI brains of these devices.
%As the market expands at an incredible rate all over the world, there is a rising need of fast language expansion for Spoken Language Understanding (SLU) models which are the AI brains of these devices. Multilingual technology, which allows the development of a single model for multiple languages, and transferring knowledge from a data resource to languages other than its own, is currently one of the best solutions to meet the increased language expansion needs. %However, as languages differ from each other in various aspects from lexicon to syntax, an interesting question that needs to be addressed is to what degree multilingual techniques can blur the language borders.
The task of SLU is usually divided into two sub-tasks, namely intent classification (IC), which identifies the intent of an user's utterance; and slot filling (SF), which extracts semantic constituents from the utterance. Consider an annotated utterance from the ATIS dataset \cite{atis}: 
\begin{quote}
    \textbf{city}~~~~~~ [$_{\bf{O}}$~where] [$_{\bf{O}}$~is] [$_{\bf{B-airport\_code}}$~MCO]
\end{quote}
 The SF sub-task should classify ``where'' and ``is'' as ${\bf{O}}$ (i.e. Other); and ``MCO'' as ${\bf{B-airport\_code}}$, while the IC sub-task should identify \textbf{city} as the intent. Current state-of-the-art SLU models are mostly DNN-based joint models of the two sub-tasks \cite{Liu2016AttentionBasedRN,do19,chen19}. These models usually contain two individual decoders to detect slot and intent labels on top of a shared encoder. As in many other NLP fields, the BERT encoder-decoder architecture has shown its strong ability in capturing contextual information from data sources to improve SLU performance \cite{chen19}. For common SLU use cases, the BERT encoder is pre-trained on a huge amount of unlabeled texts and then fine-tuned on SLU training data.
 
Since the voice-controlled device market has been expanding at an incredible rate all over the world, there is a rising need of fast language expansion for SLU models. Multilingual technology, which allows the development of a single model for multiple languages, and transferring knowledge from a data resource to languages other than its own, is currently one of the best solutions to meet the increased need.
 Traditionally, an SLU model is trained on supervised monolingual data leading to the fact that a virtual assistant often can use only one language within a working session. In contrast, a multilingual SLU model trained on supervised multilingual data, can provide the virtual assistant the ability to talk in multiple languages within a working session. Moreover, from a development perspective, multilingual modeling helps not only to reduce the number of models to build, but also to reduce supervised data needs by transferring knowledge across languages. However, as languages differ from each other in various aspects from lexicon to syntax, the cross-language knowledge transfer of the current multilingual techniques may still be limited. This raises the questions of: i) what an ideal cross-language knowledge transfer would be; ii) what a naive cross-language knowledge transfer would be; and iii) to what degree a multilingual model can transfer knowledge across languages.
 
 
 %what an ideal multilingual performance would be. Let us consider three models trained on the \textit{same} amount of knowledge (represented as training data): i) A multilingual model $xy$ which has 50\% of the training data in language $X$, and the other 50\% in language $Y$; ii) A monolingual model $x$ which has 100\% of the training data in language $X$; iii) A monolingual model $y$ which has 100\% of the training data in language $Y$. In an \textit{ideal} case, in which the language border between $X$ and $Y$ is completely blurred, model $xy$ should have similar performance on both languages $X$ and $Y$ as the respective monolingual models $x$ and $y$.

As one of the most successful multilingual techniques recently, multilingual BERT (mBERT) \cite{mBERT} is being used more and more commonly in natural language processing models in both zero-shot\footnote{The model is trained in one language and tested on another.} and multilingual\footnote{The model is trained on multiple languages.} scenarios \cite{wu-dredze-2019-beto,multiatis++}. Since mBERT is trained without any cross-lingual objectives and does not leverage aligned data, its strong cross-lingual abilities are surprising and have, in turn, spurred research aiming to understand why it is able to achieve them %Detailed analyses towards this question suggest that mBERT is able to create multilingual representations%, though performance differs across language pairs, depending on the similarity of the languages in question 
 \cite{pires2019multilingual}. In this paper, we, however, focus on addressing the question of to what degree it can blur the language borders in the \textit{multilingual} SLU setting by comparing its ability to transfer knowledge across languages with the ideal and naive cases. In addition, as mBERT is pre-trained for general purpose, we are also interested in how to improve its multilinguality for the particular use case of multilingual SLU.

%In addition, we propose a novel adversarial fine-tuning model architecture for mBERT-based SLU to approach closer to the ideal case.

Our contribution in this paper is two-fold: \textit{First}, by performing a wide range of experiments with bilingual and trilingual SLU models, we show that although mBERT is substantially good in blurring language borders even on distant language groups, there is still a gap to the ideal multilingual performance. \textit{Second}, we propose a novel adversarial model architecture to learn language-shared and language-specific representations on top of mBERT representations when fine-tuning on SLU data. The experimental results prove that our proposed approach can 
narrow the gap to the ideal multilingual performance.

 
 %Currently, mostly DNNs are explored for SLU, which model IC and SF jointly to leverage the interaction between the two subtasks (e.g. \newcite{Liu2016AttentionBasedRN}, \newcite{do19},  \newcite{chen19}). In particular, joint SLU models based on BERT \cite{mBERT} have been shown to give strong results (e.g. \newcite{chen19}).

%Recently, there has been a growing body of work investigating cross-lingual approaches to SLU which aim to decrease data requirements for building a SLU model in a (resource-poor) target language by leveraging data from one or more source languages. Common approaches include machine translation of source data \cite{gaspers2018} and pre-training a model on one or several source languages, and subsequently applying it directly (zero-shot)  \cite{pires2019multilingual} or first fine-tuning it on target language data \cite{do-gaspers-2019-cross}. Due to the growing interest in this topic, mutilingual datasets have been created for evaluating corresponding approaches by translating English SLU data into different target languages, yielding parallel SLU datasets (e.g. \newcite{multiatis++}).

%With the success of multilingual BERT (M-BERT) \cite{mBERT}, fine-tuning M-BERT for a target task has become a common approach to several NLP tasks. In particular for zero-shot scenarios fine-tuning M-BERT on task source language data and then applying it on task target language data has been shown to give strong results across several tasks \cite{wu-dredze-2019-beto}, including SLU \cite{multiatis++}. Since M-BERT is trained without any cross-lingual objective and doesn't leverage aligned data, its strong cross-lingual abilities are surprising and have, in turn, spurred research aiming to understand why it is able to achieve them. Detailed analyses towards this question suggest that M-BERT is able to create multilingual representations, though performance differs across language pairs, depending on the similarity of the languages in question \cite{pires2019multilingual}. 

%In this paper, we explore to which degree representations in multilingual BERT-based SLU models generalize across languages and how multilingual representation learning for SLU can be improved. While multilingual representation learning of M-BERT itself has been investigated extensively, to the best of our knowledge it has not yet been explored for BERT-based SLU models. Towards this goal, we first propose a new method for probing a model's multilingual abilities, which is applicable not just for SLU, but also for other NLP downstream tasks. For this purpose, we make use of parallel data, i.e. the MultiATIS++ dataset in case of SLU \cite{multiatis++}. Parallel data allows us to construct multilingual datasets by replacing (disjoint) subsets of utterances in the training data of a target language by their corresponding translations from other languages. Since the information w.r.t. to the SLU task at hand remains unchanged due to utterance parallelity, we expect a (strong) ability to create multilingual representations if performance of a model trained on such a constructed multilingual dataset comes close to that of a model trained on the original monolingual training data. 

%With this probing method we investigate multilingual representation learning in BERT-based joint SLU models for IC and SF. In addition, aiming to improve multilingual representation learning, we develop an adversarial approach to BERT-based SLU which aims to account for linguistic differences across languages by dividing the model into language-shared and language-specific representations. While adversarial approaches to cross-lingual transfer learning for slot filling have been explored using LSTMs (\newcite{8990095}, \newcite{chen-etal-2019-multi-source}), to the best of our knowledge BERT-based joint models for IC and SF have not yet been investigated and detailed analysis on multilingual representation learning abilities are still missing.  

%We present empirical results on the MultiATIS++ and a real-world dataset investigating multilingual learning with two groupings of languages, where one includes a distant language pairing, i.e. English, German, Spanish and English, German, Japanese. Our results show that



%In the past years, Alexa has been localised to 12 different countries including 10 different languages.
%At the same time we observe an increasing number of bilingual Alexa house holds.
%Solving the problem of Spoken Language Understanding (SLU), namely Intent Classification (IC) and Slot Filling (SF) for multiple languages is one important tasks of Alexas voice assistant.
%With the increasing need to support the same Alexa functionality across different languages the approach of a multi-lingual SLU model providing the same functionalities all-in-one becomes more attraction.
%To tackle this problem, recent efforts focus on the approach of Cross Lingual Transfer Learning (CLTI) to overcome the need of labeled training data for each target language.
%Typical approaches focus on a bilingual transfer learning model, where models are pre-trained on supervised data from a single source language and then either apply it directly on a target language (zero shot) \cite{pires2019multilingual}, or fine-tune it on a smaller labeled data set in the target language \cite{cross_quyn_gasp}. 
%
%However, in a large-scale environment we typically have labeled data for all languages available covering training utterances for the same or different Alexa functionalities. 
%Hence, a straight forward method is to utilize all of the data when transferring to another language.
%Another benefit of the multi-lingual approach is that the resulting SLU model provides Alexa feature support and feature parity for more than one language at a time, and at the same time only one model needs to be maintained.
%This becomes more and more important considering several bi-lingual households not only in Europe.
%
%In this paper, we investigate if we can loose the border controls between different languages, respectively treat supervised training data language-indepedent during the process of fine tuning for the purpose of SLU.
%We run experiments on parallel language specific data sets to identify if the model, e.g. can treat German labeled data as English labeled data and vise versa.
%We investigate the opportunity to reach similar individual language model performance with a Multi-Lingual Transfer Learning (MLTL) approach compared to fine-tune on each language in a mono-lingual setup.
%For the comparison both models use the same amount of training data, MLTL approach with a mixed language labeled data and language specific for mono-lingual.
%
%In this paper, we investigate the opportunity to reach similar individual language model performance with a Multi-Lingual Transfer Learning (MLTL) approach compared to train each language in a mono-lingual setup.
%when fine-tuning on a multi-lingual training set compared to fine-tune each language individually (mono-lingual) with the same amount of data.
%
%
%We compare three/two?? different approaches/model architectures.
%First, we experiment with Multilingual BERT (M-BERT) as a baseline model, re-leased by \cite{mBERT} as a single language model pre-trained on the concatenation of mono-lingual Wikipedia corpora from 104 languages.
%Second, we propose a language-adversarial training approach to allow for extracting language invariant features with respect to the language shift.
%Model performance is evaluated on an extended ATIS data set \cite{atis} and Alexa in-house data.
%We consider bi-lingual and tri-lingual models, considering the need in our Production systems.
%???The proposed language-adversarial approach beats all baseline models and also shows lower training times....

==> COLING 2020 (1) (6)/sections/introduction.tex <==
\section{Introduction}
In the past years, Alexa has been localised to 12 different countries including 10 different languages.
At the same time we observe an increasing number of bilingual Alexa house holds.
Solving the problem of Spoken Language Understanding (SLU), namely Intent Classification (IC) and Slot Filling (SF) for multiple languages is one important tasks of Alexas voice assistant.
With the increasing need to support the same Alexa functionality across different languages the approach of a multi-lingual SLU model providing the same functionalities all-in-one becomes more attraction.
To tackle this problem, recent efforts focus on the approach of Cross Lingual Transfer Learning (CLTI) to overcome the need of labeled training data for each target language.
Typical approaches focus on a bilingual transfer learning model, where models are pre-trained on supervised data from a single source language and then either apply it directly on a target language (zero shot) \cite{pires2019multilingual}, or fine-tune it on a smaller labeled data set in the target language \cite{cross_quyn_gasp}. 

However, in a large-scale environment we typically have labeled data for all languages available covering training utterances for the same or different Alexa functionalities. 
Hence, a straight forward method is to utilize all of the data when transferring to another language.
Another benefit of the multi-lingual approach is that the resulting SLU model provides Alexa feature support and feature parity for more than one language at a time, and at the same time only one model needs to be maintained.
This becomes more and more important considering several bi-lingual households not only in Europe.

In this paper, we investigate if we can loose the border controls between different languages, respectively treat supervised training data language-indepedent during the process of fine tuning for the purpose of SLU.
We run experiments on parallel language specific data sets to identify if the model, e.g. can treat German labeled data as English labeled data and vise versa.
We investigate the opportunity to reach similar individual language model performance with a Multi-Lingual Transfer Learning (MLTL) approach compared to fine-tune on each language in a mono-lingual setup.
For the comparison both models use the same amount of training data, MLTL approach with a mixed language labeled data and language specific for mono-lingual.

In this paper, we investigate the opportunity to reach similar individual language model performance with a Multi-Lingual Transfer Learning (MLTL) approach compared to train each language in a mono-lingual setup.
when fine-tuning on a multi-lingual training set compared to fine-tune each language individually (mono-lingual) with the same amount of data.


We compare three/two?? different approaches/model architectures.
First, we experiment with Multilingual BERT (M-BERT) as a baseline model, re-leased by \cite{mBERT} as a single language model pre-trained on the concatenation of mono-lingual Wikipedia corpora from 104 languages.
Second, we propose a language-adversarial training approach to allow for extracting language invariant features with respect to the language shift.
Model performance is evaluated on an extended ATIS data set \cite{atis} and Alexa in-house data.
We consider bi-lingual and tri-lingual models, considering the need in our Production systems.
???The proposed language-adversarial approach beats all baseline models and also shows lower training times....
\label{introduction}




==> COLING 2020 (1) (6)/sections/method.tex <==
% !TEX root = ../multilingual_DNN_coling.tex
\section{BERT-based multilingual SLU models}
\label{lbl:method}
%\subsection{Probing method for multilingual representation learning}
In this section, we describe the two multilingual SLU models evaluated in this paper. %The first model, which is a simple multilingual approach, uses a BERT encoder to learn language-shared representations. The second model, which is an  adversarial approach, makes use of a BERT encoder and multiple CNN encoders to learn language-shared and language-specific representations, respectively. 

%First, we present a standard approach, in which a BERT encoder is used as the model's language-shared feature extractor. Second, we describe an adversarial approach, in which the single shared feature extractor is extended with $n$ language-specific feature extractors.
\subsection{SLU as a downstream task of BERT}
\label{slu-bert}
\begin{figure}[h]
\centering
\includegraphics[width=10cm]{figs/coling2020_bert1.png}
\caption{A standard BERT-based SLU model architecture.}
\label{fig:bert_slu}
\end{figure}
Fig. \ref{fig:bert_slu} shows our BERT-based SLU model architecture. 
Like \newcite{chen19} and \newcite{gaspers2020data}, our model consists of a BERT encoder receiving sub-word and position embedding layers as inputs, an IC decoder to identify intent labels, and an SF decoder to predict slot labels. In particular, given an utterance $u$, the final hidden states of the tokens $h_1\ldots h_T$ produced by the encoder, are used as the token representations. The sentence presentation, denoted by ${s_u}$, is computed from $h_1\ldots h_T$ by using max-pooling.

${s_u}$ is passed through the IC decoder, which is composed from  a feed-forward of 2 dense layers ($\text{FFN}^I$) and a linear output layer to predict the intent:
\begin{equation}
\begin{split}
\hat{s}_u  =  \text{FFN}^I(s_u) \\
p^i(.|u)  =  \text{softmax}({\bf W}^I\hat{s}_u + b^I)
\end{split}
\label{eq:pri}
\end{equation}

$h_1\ldots h_T$ are passed through the SF decoder, which is composed from a position-wise feed-forward of 2 dense layers ($\text{FFN}^S$) and a CRF layer on top \cite{zhou-xu-2015-end} to predict slot labels:
\begin{equation}
\begin{split}
\hat{h}^t  =  \text{FFN}^S(h^t) \\
\end{split}
\label{eq:pri}
\end{equation}
The CRF layer takes $\hat{h}^t$ as inputs, and estimates a transition matrix modeling the dependence among adjacent labels. The slot labels are predicted by the traditional Viterbi decoding. 

The model is trained by optimizing the joint loss $L  =  L_i + L_s$ where $L_i$ and $L_s$ are the cross entropy loss for intent identification and the CRF loss for slot classification, respectively.

As a downstream task of BERT, the embedding and encoder layers are initialized by a pre-trained BERT language model. The full model is  trained on a supervised SLU dataset.

%The BERT encoder is used to learn token and sentence representations, which are then passed to the IC and SF decoders, respectively. Similarly to other downstream tasks, the embeddings and encoder are initialized by the parameters of a trained BERT language model. In our model, the IC decoder is a standard two-layer perceptron classifier with softmax activation function at the output layer.  Meanwhile, the SF decoder uses a CRF layer on top of two dense layers to leverage the sequential information of slot labels. During training, the losses of IC and SF are optimized jointly with equal weights.

%Depending on the 


\subsection{A simple approach for multilingual modeling}
\label{lbl:method:standard}
Thanks to the strong multilingual abilities of mBERT, we simply use mBERT for the model described in \ref{slu-bert} to obtain a simple multilingual SLU model. In particular, the embedding and encoder layers are initialized by the parameters of a pre-trained mBERT. The full model is then trained on a mix of supervised data from multiple languages.

%for the SLU task using a mixed training set which contains supervised data from each of our target languages.



%For training multilingual SLU models, we use pre-trained mBERT \cite{mBERT}, whose modules including subword embeddings, position embeddings and BERT encoder were pre-trained on a large amount of unlabelled texts in multiple languages. We fine-tune the full model for the SLU task using a mixed training set which contains supervised data from each of our target languages.


\subsection{An adversarial approach for multilingual modeling}
\label{lbl:adv}
\begin{figure}[h]
\centering
\includegraphics[width=15cm]{figs/coling2020_adv_new.png}
\caption{An adversarial model architecture for BERT-based trilingual SLU.}
\label{fig:adv_bert_slu}
\end{figure}

The simple multilingual model, as described in Sec. \ref{lbl:method:standard}, learns language-shared token and sentence representations from multilingual training data via its BERT encoder. However, as languages differ from each other in various aspects, using only language-shared representations may be \textit{not} enough to reach the optimal performance in all of the target languages. Our hypothesis is that encouraging a model to learn \textit{both language-shared and language-specific representations} will narrow the gap to the ideal multilingual SLU model in which knowledge can be transferred freely across language borders.

Motivated by the success of adversarial approaches in natural language processing, we propose a novel BERT-based  adversarial SLU model using a single BERT encoder to learn language-shared representations across all target languages, and  multiple CNN encoders to learn language-specific representations for each of the target languages. The language-shared and language-specific representations are concatenated before being fed to the IC and SF decoders. The full model is trained via an adversarial training strategy. Fig. \ref{fig:adv_bert_slu} show our model architecture for a trilingual use case.

In a general use case targeting $N$ languages $l_1, \ldots , l_N$, the model has $N+3$ encoders:  First, it contains a BERT encoder denoted by $enc_{bert}$, which can be initialized by pre-trained BERT parameters. %, which is pre-trained on unlabelled texts. 
Second, we use $N$ 1-layer CNN encoders to learn language-specific representations for $l_1, \ldots , l_N$, denoted by $enc_{l_1} , \ldots , enc_{l_N}$, respectively. Third, an 1-layer CNN encoder denoted by $enc_{lang}$ is used to learn features for predicting the language of the input utterance. Finally, another 1-layer CNN encoder denoted by $enc_{shared}$ is used to learn shared representations across languages. 

Given utterance $u$ as input, the final hidden states of the tokens $h_1\ldots h_T$ produced by $enc_{bert}$ are used as the inputs of the CNN encoders. Each CNN encoder, $enc$, generates its token and sentence representations, namely $h^{enc}_t$ and $s^{enc}_u$:
\begin{equation}
\begin{split}
h^{enc}_1, \ldots, h^{enc}_T = \text{CNN}^{enc}(h_1,\ldots,h_T) \\
s^{enc}_u = \text{max\_pooling}(h^{enc}_1,\ldots ,h^{enc}_T)
\end{split}
\label{eq:pri}
\end{equation}

In addition to the normal IC and SF decoders, we add two more decoders: a language predictor and a language discriminator. Each of the additional decoders consists of a feed-forward of 1 dense layer ($\text{FFN}$) and a linear output layer to predict the language of $u$. 

The language predictor receives $s^{enc_{lang}}_u$, which is the sentence representation computed by $enc_{lang}$, as input, and outputs a language distribution $p^P$:
\begin{equation}
\begin{split}
\hat{s}^{P}_u  =  \text{FFN}^P(s^{enc_{lang}}_u) \\
p^P(.|u)  =  \text{softmax}({\bf W}^P\hat{s}^{P}_u + b^P)
\end{split}
\end{equation}

The language-specific token and sentence representations are computed as following:
\begin{equation}
\begin{split}
h^{specific}_t  = \sum_{l \in {l_1, \ldots , l_N}} h^{enc_l}_t * p^P(l|u) \\
s^{specific}_u  = \sum_{l \in {l_1, \ldots , l_N}} s^{enc_l}_u * p^P(l|u) 
\end{split}
\end{equation}

The combined token and sentence representations are computed as following:
\begin{equation}
\begin{split}
h^{combined}_t  =  h^{specific}_t \oplus h^{enc_{shared}}_t  \\
s^{combined}_u  =  s^{specific}_u  \oplus s^{enc_{shared}}_u
\end{split}
\label{eq:com}
\end{equation}

The combined token and sentence representations are used as inputs to the IC and SF decoders as described in Sec. \ref{slu-bert}.

The language discriminator receives the sentence representation from $enc_{shared}$ as input, and also predicts the language distribution of $u$ as the language predictor:
\begin{equation}
\begin{split}
\hat{s}^{D}_u  =  \text{FFN}^D(s^{enc_{shared}}_u) \\
p^D(.|u)  =  \text{softmax}({\bf W}^D\hat{s}^{D}_u + b^D)
\end{split}
\end{equation}
However, the discriminator is trained adversarially to confuse the system about the distinction between languages. This encourages the model to learn shared-language representations.
%which are 1-layer perceptron classifiers with softmax activation function in the output layers. 
%The language predictor receives the sentence representations from $enc_{lang}$ as inputs, and predicts the language distributions of the input data: $(p_X, p_Y, p_Z)$ which will be used to compute the language-specific features. Meanwhile, the language discriminator receives the sentence representations from $enc_{shared}$ as inputs and also predicts language distributions. However, the discriminator is trained to fool the system such that the languages becomes indistinguishable. 

We use CRF loss for the SF task, denoted by $L_s$. Meanwhile, for the IC decoder, language predictor, and language discriminator, we use cross-entropy losses denoted by  $L_i, L_p$ and $L_d$, respectively. The full model is trained by an adversarial training strategy as shown in Alg. \ref{alg:adv}. 
%We denote the token representations and sentence representations outputted by encoder $enc$ as $out^{tok}(enc)$, and $out^{sen}(enc)$, respectively. Meanwhile, the input of $enc$ is denoted by $in(enc)$.  

%The token representations of $enc_{bert}$ are used as the inputs for the CNN encoders (see Eq. \ref{eq:enc}).
%\begin{equation}
%    in(enc_X) = in(enc_Y) = in(enc_Z) = in(enc_{lang}) = in(enc_{shared}) =  out^{tok}(enc_{bert}) 
%    \label{eq:enc}
%\end{equation}

%The language-specific token and sentence representations are computed as in Eq. \ref{eq:pri}.
%\begin{equation}
%\begin{split}
%tok_{lang-specific}  =  \sum_{l \in {X, Y, Z}} out^{tok}(enc_l) * p_l \\
%sen_{lang-specific}  =  \sum_{l \in {X, Y, Z}} out^{sen}(enc_l) * p_l
%\end{split}
%\label{eq:pri}
%\end{equation}

%The combined token and sentence representations are computed as in Eq. \ref{eq:com}.
%\begin{equation}
%\begin{split}
%tok_{combined}  =  tok_{lang-specific} \oplus out^{tok}(enc_{shared}) \\
%sen_{combined}  =  sen_{lang-specific} \oplus out^{sen}(enc_{shared})
%\end{split}
%\label{eq:com}
%\end{equation}


%in(enc_X) = in(enc_Y) = in(enc_Z) = in(enc_{lang}) = in(enc_{shared}) =  out^{tok}(enc_{bert}) \\

%\begin{algorithm}%[H]
%\SetAlgoLined
%\KwInput{SLU training data in multiple languages with intent, slot and language labels. $\alpha_d, \alpha_i, \alpha_s, \alpha_p, \beta_d$ are model hyper-parameters.}

% \While{not converge}{
%  Randomly generates some data batches \\
%  Computes $L_1 = \alpha_d L_d$ \\
%  Optimizes $L_1$ and updates model weights \\
%  Randomly generates some data batches \\
%  Computes $L_2 = \alpha_i L_i + \alpha_s L_s + \alpha_p L_p - \beta_d L_d$   \\
%  Optimizes $L_2$ and updates model weights \\
% }
% \caption{Adversarial training strategy}
%   \label{alg:adv}
%\end{algorithm}

\begin{algorithm}%[H]
\SetAlgoLined
\KwInput{SLU training data in multiple languages with intent, slot and language labels. $\alpha_d, \alpha_i, \alpha_s, \alpha_p, \beta_d$ are model hyper-parameters.}
Task 1: To optimize $L_1 = \alpha_d L_d$ \\
Task 2: To optimize $L_2 = \alpha_i L_i + \alpha_s L_s + \alpha_p L_p - \beta_d L_d$   \\
 \While{number\_of\_epochs(Task 1) $<$ K or  number\_of\_epochs(Task 2) $<$ K}{
    Randomly pick a task $j$ ($j \in \{1, 2\}$) \\
    %\eIf {$i==1$} {
        Generates a mini-batch for Task j  \\
        Updates model weights to optimize $L_j$
    %} {
    %    Generates a mini-batch for Task 2 \\
    %    Updates model weights to optimize $L_2$
    %}
 }
 \caption{Adversarial training strategy}
   \label{alg:adv}
\end{algorithm}



\section{An ideal multilingual SLU performance vs. a naive multilingual SLU performance}
\label{lbl:ideal-flawed}
To address the question of to what degree knowledge can be transferred across languages in multilingual SLU, in this section, we define an ideal and a naive multilingual performance. Let us consider a multilingual SLU model $\mathcal{M}$ for $n$ languages $l_1, l_2, \ldots l_n$. % and a training set $\bf D$ in which each annotated utterance can be in one of the $n$ target languages. % and an evaluation metric $eval(\mathcal{M}, l)$ which evaluates the performance of $\mathcal{M}$ on language $l$. 
 We use the following notations:
\begin{itemize}
    \item ${\bf D}$: a training set, in which each annotated utterance can be in one of the $n$ target languages.
    \item ${\bf D}^l$: The monolingual version of $\bf D$ in language $l$. That means ${\bf D}^l$ and ${\bf D}$ contain the same utterances, but all of the utterances in ${\bf D
}^l$  are in $l$ only.
    \item ${\bf d}^l$: A subset of $\bf D$ containing all utterances which are in language $l$.
    \item $\mathcal{M(\bf T)}$: Model $\mathcal{M}$ trained on dataset $\bf T$.
    \item $eval(\mathcal{M}, l)$: An evaluation metric  evaluating the performance of $\mathcal{M}$ on the test set of language $l$.
    \item $\mathcal{M'}$: A monolingual SLU model.
\end{itemize}
Given ${\bf D}$, the average performance of $\mathcal{M}$ on the target languages is computed in Eq. \ref{eq:mavg}.
\begin{equation}
\text{avg}_\mathcal{M} = \frac{1}{n}*\sum_{l \in  l_1, l_2, \ldots l_n}eval(\mathcal{M}({\bf D}), l)
\label{eq:mavg}
\end{equation}
\subsection{Ideal case}
Ideally, the language borders are completely blurred and knowledge can be transferred freely across different languages. Given ${\bf D}$,  for each target language $l$, the multilingual performance ($eval(\mathcal{M({\bf D})}, l)$) should \textit{reach or outperform} the performance of a monolingual model trained on a similar amount of knowledge ($eval(\mathcal{M'}({{\bf D}^l}), l)$). For example, let us consider three models trained on the \textit{same} amount of knowledge (represented as training data): i) A multilingual model $xy$ which has 50\% of the training data in language $X$, and the other 50\% in language $Y$; ii) A monolingual model $x$ which has 100\% of the training data in language $X$; iii) A monolingual model $y$ which has 100\% of the training data in language $Y$. In an \textit{ideal} case, model $xy$ should have similar performance on languages $X$ and $Y$ as the respective monolingual models $x$ and $y$. 

For the rest of this paper, we will refer to $eval(\mathcal{M'}({{\bf D}^l}), l)$ as the Ideal baseline on language $l$ given $\bf D$. We also define an Ideal baseline for the average performance on the target languages in Eq. \ref{eq:mideal}. Comparing $avg_\mathcal{M}$ with $avg_{ideal}$ will indicate how close $\mathcal{M}$ is to the ideal performance.

\begin{equation}
\text{avg}_{ideal} = \frac{1}{n}*\sum_{l \in  l_1, l_2, \ldots l_n} eval(\mathcal{M'}({{\bf D}^l}), l)
\label{eq:mideal}
\end{equation}
\subsection{Naive case}
Given ${\bf D}$, in a naive multilingual case, for each target language $l$, the multilingual performance   ($eval(\mathcal{M({\bf D})}, l)$) \textit{cannot outperform} the monolingual model trained on the subset of its training data containing utterances which are in $l$ ($eval(\mathcal{M'}({{\bf d}^l}), l)$). That means, the model performance in a language can not be improved by adding more training utterances from other languages. Let us reconsider the previous example. In a naive case, in which the language border between $X$ and $Y$ is completely closed, the performance of model $xy$ on  languages $X$ and $Y$ should be worse than the respective monolingual models $x$ and $y$. 

For the rest of this paper, we will refer to $eval(\mathcal{M'}({{\bf d}^l}), l)$ as the Naive baseline on language $l$ given $\bf D$. A Naive baseline for the average performance on the target languages can be found in Eq. \ref{eq:mflawed}. Comparing $avg_\mathcal{M}$ with $avg_{naive}$ will indicate how far $\mathcal{M}$ is from being naive.



\begin{equation}
\text{avg}_{naive} = \frac{1}{n}*\sum_{l \in  l_1, l_2, \ldots l_n} eval(\mathcal{M'}({{\bf d}^l}), l) 
\label{eq:mflawed}
\end{equation}
%where $\mathcal{M'}$ is a monolingual SLU model.

%We consider a model as \textit{ideal} when it has comparable performance as the monolingual model trained on a similar amount of knowledge, in any of the target languages (see Equation \ref{eq:ideal}). That means the language borders are completely blurred, and the knowledge can be transferred freely across different languages. In contrast, we consider a model as \textit{flawed} when for each language $l$, it cannot outperform the monolingual model trained on the subset of its training data containing utterances which are in $l$ (see Equation \ref{eq:flawed}). In this case, the model performance in a language can not be improved by adding more training utterances from other languages. 
%\begin{equation}
%\begin{split}
%eval(\mathcal{M}_{ideal}({\bf D}), l)  \approx eval(\mathcal{M'}({\bf D}^l), l) \quad  \forall l \in  l_1, l_2, \ldots l_n
%\end{split}
%\label{eq:ideal}
%\end{equation}
%\begin{equation}
%\begin{split}
%eval(\mathcal{M}_{flawed}({\bf D}), l)  \leq^* eval(\mathcal{M'}({\bf d}^l), l) \quad  \forall l  \in  l_1, l_2, \ldots l_n
%\end{split}
%\label{eq:flawed}
%\end{equation}
%where $\mathcal{M'}$ is a monolingual SLU model, and  $\leq^*$ refers to an ``is worse than or equal to" operator.

%The average performance of $\mathcal{M}$, the ideal average performance and the flawed average performance on the target languages denoted by $mul_\mathcal{M}$, $mul_{ideal}$, and  $mul_{flawed}$, respectively, are computed by:
%\begin{equation}
%\begin{split}
%mul_\mathcal{M} = \frac{1}{n}*\sum_{l \in  l_1, l_2, \ldots l_n} %eval(\mathcal{M}({\bf D}), l) \\
%mul_{ideal} = \frac{1}{n}*\sum_{l \in  l_1, l_2, \ldots l_n} eval(\mathcal{M'}({{\bf D}^l}), l) \\
%mul_{flawed} = \frac{1}{n}*\sum_{l \in  l_1, l_2, \ldots l_n} %eval(\mathcal{M'}({{\bf d}^l}), l) 
%\end{split}
%\end{equation}

%Comparing $avg_\mathcal{M}$ with $avg_{ideal}$, and $avg_{flawed}$ will indicate how multilingual $\mathcal{M}$ is.

%Note that, for the rest of the paper, we will refer to $eval(\mathcal{M'}({{\bf D}^l}), l)$ and $eval(\mathcal{M'}({{\bf d}^l}), l)$ as the Ideal and Flawed performances on language $l$, respectively.



==> COLING 2020 (1) (6)/sections/results.tex <==
% !TEX root = ../multilingual_DNN_coling.tex
%\section{Results}
\subsection{Performance on real-world SLU data}
We investigated performance of our SLU models on real-world data to explore the impact on a real-world scenario. Since parallel data were not available for these experiments, we cannot provide performance in relation to an Ideal baseline. Instead, we use the Naive baseline and determine the relative gain obtained by the two multilingual SLU models. The results for two language triples (EN, DE, ES) and (EN, DE, JA) are presented in Table \ref{results_alexa}.
\begin{table}[ht]
\centering
\resizebox{0.8 \textwidth}{!} {
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|} %l|l|l|}
\hline
\multirow{2}{*}{\textbf{Exp.}} & \multirow{2}{*}{\textbf{Target}} &  \multirow{2}{*}{\textbf{Model}}& \multicolumn{3}{|c|}{\textbf{Music domain}} & \multicolumn{3}{|c|}{\textbf{Books domain}} & \multicolumn{3}{|c|}{\textbf{Video domain}} \\%&  \multicolumn{3}{|c|}{\textbf{Average}} \\
%\hline
\cline{4-12} 
&&&$\Delta$ SemER&$\Delta$ SF F1&$\Delta$ IC acc.&$\Delta$ SemER&$\Delta$ SF F1&$\Delta$ IC acc.&$\Delta$ SemER&$\Delta$ SF F1&$\Delta$ IC acc.\\%&SemER&SF F1&IC acc.\\
\hline
\hline
\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{EN-DE-ES}}}
&\multirow{2}{*}{EN} &Multi-lang.&-24.14 &+7.18 &+3.07 & -16.53&+2.64 &+3.62&-10.41 &+3.18 &+3.98\\%&-16.77 &+4.31 &+3.54\\
& & Lang.-adv.&-24.81&+7.03 & +3.34& -29.84&+4.58 & +7.69&-18.8&+6.21 &+4.77 \\%&-23.76&+5.91 & +5.22\\
\cline{2-12} 
&\multirow{2}{*}{DE} &Multi-lang.&-20.06 & +5.24& +3.19& -9.2 &+0.68 &+5.62&-16.00 &+6.6 &+3.48\\%&-15.23 &+4.07 &+4.06\\
& & Lang.-adv.&-23.89& +6.1& +3.46&-28.02 &+3.23 &+11.24&-25.22 &+10.48 &+4.46\\%&-25.64& +6.44& +6.27\\
\cline{2-12} 
&\multirow{2}{*}{ES} &Multi-lang.&-27.85 &+9.29 &+3.13 & -18.25&+2.1 &+8.45&-15.5 &+5.41 &+4.97\\%& -14.04&+5.52 &+5.44\\
& & Lang.-adv.&-29.18& +9.6&+3.18 &-29.17 &+4.63 &+12.44 &-20.44& +7.81&+5.97\\% &-20.1&+7.04 & +6.87\\
\cline{2-12} 
&\multirow{2}{*}{Avg.} &Multi-lang. & -24.02 & +7.24 & +3.13 &  -14.66 &+1.81 &+5.89 & -13.97 & +4.92 &+4.14 \\% &&  &  \\
& & Lang.-adv.& \textbf{-25.96} & \textbf{+7.58 }& \textbf{+3.33} & \textbf{-29.01} & \textbf{+4.15} & \textbf{+10.46} & \textbf{-21.49} & \textbf{+8.17}&\textbf{+5.07} \\% &&  & \\
\hline
\hline
\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{EN-DE-JA}}}
&\multirow{2}{*}{EN} &Multi-lang.& -19.5&+5.98 & +2.86&-12.88 &+1.15 &+4.07& -5.67&+1.96 &+3.18\\%& -12.33& +2.99&+3.36\\
& & Lang.-adv.&-25.32&+7.37 & +3.28&-27.4 &+4.32 &+6.56 &-17.3&+5.28 & +4.77\\%&-22.69& +5.63& +4.83\\
\cline{2-12} 
&\multirow{2}{*}{DE} &Multi-lang.& -20.67&+5.17 &+3.08 &-8.9 &+0.53 &+3.98& -10.4& +4.4&+2.07\\%&-13.06 &+3.33 &+3.08\\
& & Lang.-adv.&-24.66& +6.67& +3.24&-23.56 & +2.7&+9.6 &-20.89&+8.14 & +4.46\\%&-22.81& +5.74& +5.73\\
\cline{2-12} 
&\multirow{2}{*}{JA} &Multi-lang.&-27.82 &+13.36 &+2.28 & -3.9&-3.41 &+6.49&-0.1 &-6.5 &+3.18\\%&-9.8 &+1.26 &+3.89\\
& & Lang.-adv.&-31.9& +14.49& +2.81&-13.67 &+0.77 &+12.26 &-17.93&+2.47 &+6.93 \\%&-25.12& +8.41& +7.2\\
\cline{2-12} 
&\multirow{2}{*}{Avg.} &Multi-lang. & -22.66 & +8.17 & +2.74 & -8.56  & -0.58 & +4.85& -5.39 & -0.05 & +2.81 \\%&&  &  \\
& & Lang.-adv.&\textbf{ -27.29} & \textbf{+9.51} & \textbf{+3.11 }&  \textbf{-21.54}& \textbf{+2.60} & \textbf{+9.47} & \textbf{-18.71} &\textbf{+5.30} & \textbf{+5.39}  \\%&&  & \\
\hline
\hline

\end{tabular}
}
\caption{Relative change in semantic error rate (SemER), intent classification accuracy and slot F1 for multilingual and language-adversarial training compared to the Naive baseline. Negative numbers indicate better performance for SemER, while positive numbers indicate better performance for slot F1 and intent classification accuracy.} 
\label{results_alexa}
\end{table}


Overall, multilingual models improves performance over the Naive baselines. In particular, the only drops in performance are observed for slot filling in JA with Multi-lang. on two out of the three domains. This drop may be attributed to JA being linguistically distant to the other languages, which are all from the European language family. The highest relative gain is up to 27.29\% in avg. SemER obtained with Lang.-adv.

Between the two multilingual models, our proposed model, Lang.-adv. outperforms Multi-lang. in all of the three domains. While the relative gains in avg. SemER of Multi-lang. fluctuate between 5.39\% and 24.02\%, those of Lang.-adv. range between 18.71\% to 29.01\%. Moreover, unlike the standard multilingual approach, Lang.-adv. models do not yield drops when the distant language JA is included in training. In fact, their relative SemER reductions for JA range from 13.67\% to 31.9\%. Thus, in particular, when distant languages are included in multilingual training, dividing the model into language-shared and language-specific parts seems to be beneficial. Taken together, the results indicate that our proposed adversarial architecture improves performance over the standard BERT-based approach not just on academic benchmark datasets, but also on real-world SLU data.
%With Multi-lang. model, as can be seen, the gains over Naive baseline are not consistent across domains for JA. 
%While besides these two drops, Multi-lang. performance also increases for JA vs. Naive baseline, the gains are on average lower than for the European languages, i.e. on average, a relative reduction in SemER of 9.8\% is achieved for JA, while gains range between 12.33\% and 16.77\% for the three European languages. Here, performance differs across scenarios. In particular, as expected, higher reductions in SemER are achieved for EN and DE when trained together with the European language ES compared to joint training with the distant language JA. Notably though, consistent gains are achieved also in the latter scenario, with up to 13.06\% and 12.33\% error rate reduction for DE and ES, respectively.

% The adversarial approach, on the other hand, yields consistent (large) gains over both the Naive baselines as well well as the multilingual standard approach. In particular, compared to the Naive baselines, average reductions in SemER range between 20.1\% and 25.64\% across languages. Unlike the standard multilingual approach, the adversarial model does not yield drops when the distant language JA is included in training. In fact, gains are particularly high for JA, with the relative gains in SF F1 and IC accuracy of 8.41\% and 7.2\%, respectively, being the highest across languages. Thus, in particular when distant languages are included in multilingual training, dividing the model into language-shared and language-specific parts seems to be beneficial. Taken together, the results indicate that our proposed adversarial architecture improves performance compared to standard mono- or multilingual approaches not just on Academic benchmark datasets, but also on real-world SLU data.  






==> COLING 2020 (1) (6)/sections/sota.tex <==
% !TEX root = ../multilingual_DNN_coling.tex
\section{Related Work}\label{sota}
As one of the most successful model architectures in natural language understanding recently, BERT models have been explored  in various researches for SLU \cite{chen19,multiatis++,gaspers2020data}. In these works, SLU is considered as a downstream task of a trained BERT model. In particular, after being pre-trained on a large amount of unlabelled data, the BERT embeddings and encoders are fine-tuned on supervised SLU data together with two SLU-adapted decoders for the IC and SF sub-tasks.  

%For the rest of this paper, we will refer to this as the standard BERT-based SLU approach.

Due to the fast expansion of voice-controlled device market, there has been a rising interest in cross-lingual and multilingual SLU modeling. In the former direction, supervised data from one or multiple source languages is leveraged to improve the SLU performance on a target language \cite{johnson-etal-2019-cross,do-gaspers-2019-cross,multiatis++}. In the later direction, SLU models are trained on supervised multilingual data for multiple target languages \cite{multiatis++}. To obtain a multilingual model, \newcite{multiatis++} simply initialized the embeddings and encoder of a BERT-based SLU model by mBERT's parameters, and then trained the full model on a mix of supervised datasets from multiple languages. Noticeably, the SLU model used in \newcite{multiatis++} was designed towards cross-lingual scenarios using a soft-alignment method to improve the slot projection between source and target languages. In this paper, we focus on only multilingual SLU modeling. Unlike \newcite{multiatis++}, our adversarial model is designed specially for multilingual model building.

%This is inline with one of the two multilingual models used in our experiments.

%In this paper, we focus on multilingual SLU modeling. One of the multilingual models used in our experiments is following the approach 

%The simple approach to train a multilingual model as evaluated in \newcite{multiatis++} is referred to as the simple multilingual model in our experiments.

%The standard mBERT encoder-decoder SLU architecture as in \cite{multiatis++}, is used as the base model in our experiments.

The impressive abilities of mBERT in cross-lingual and multilingual natural language understanding applications, have recently led to an increasing body of research analyzing how it is able to achieve those. For instance, \newcite{pires2019multilingual} probed the cross-linguality of mBERT using zero-shot transfer learning on morphological and syntactic tasks and found that mBERT is able to create multilingual representations. However, to the best of our knowledge, probing multilingual representation learning for downstream tasks, like SLU, and addressing the question of how far it is from the ideal expectation,  have not yet been explored in literature. 

Adversarial approaches aiming to account for linguistic differences across languages by dividing the model into language-shared and language-specific representations, have been explored for the SLU sub-tasks. Recently, \newcite{8990095} investigated the sub-tasks in isolation using BiLSTMs and focused on improving SLU for low-resource languages. Meanwhile, \newcite{chen-etal-2019-multi-source} explored BiLSTMs to improve named entity recognition which is close to the SF sub-task of SLU. In this work, instead of isolating the two sub-tasks, we propose a joint model based on mBERT for multilingual use cases. %Moreover,  detailed analyses on multilingual representation learning abilities for the existing approaches are still missing. 

%Further research has addressed the latter goal of improving SLU for languages with no or few data using cross-lingual resources. Common approaches include machine translation \cite{gaspers2018} and pre-training a model on one or several source languages (e.g. \newcite{johnson-etal-2019-cross}, \newcite{do-gaspers-2019-cross}). Selecting relevant data from several sources has been explored as well \cite{do-gaspers-2019-cross}. Currently, the most common approach to cross-lingual transfer is fine-tuning a multilingual pre-trained masked language model on task source data. In particular, approaches based on mBERT \cite{mBERT} have been shown to be effective in low-resource scenarios  \cite{wu-dredze-2019-beto,multiatis++}.



==> sections/acknowledgement.tex <==
\section{Acknowledgement}
Thanks to ...
\label{acknowledgement}


==> sections/introduction.tex <==
\section{Introduction}
In the past years, Alexa has been localised to 12 different countries including 10 different languages.
At the same time we observe an increasing number of bilingual Alexa house holds.
Solving the problem of Spoken Language Understanding (SLU), namely Intent Classification (IC) and Slot Filling (SF) for multiple languages is one important tasks of Alexas voice assistant.
With the increasing need to support the same Alexa functionality across different languages the approach of a multi-lingual SLU model providing the same functionalities all-in-one becomes more attraction.
To tackle this problem, recent efforts focus on the approach of Cross Lingual Transfer Learning (CLTI) to overcome the need of labeled training data for each target language.
Typical approaches focus on a bilingual transfer learning model, where models are pre-trained on supervised data from a single source language and then either apply it directly on a target language (zero shot) \cite{pires2019multilingual}, or fine-tune it on a smaller labeled data set in the target language \cite{cross_quyn_gasp}. 

However, in a large-scale environment we typically have labeled data for all languages available covering training utterances for the same or different Alexa functionalities. 
Hence, a straight forward method is to utilize all of the data when transferring to another language.
Another benefit of the multi-lingual approach is that the resulting SLU model provides Alexa feature support and feature parity for more than one language at a time, and at the same time only one model needs to be maintained.
This becomes more and more important considering several bi-lingual households not only in Europe.

In this paper, we investigate if we can loose the border controls between different languages, respectively treat supervised training data language-indepedent during the process of fine tuning for the purpose of SLU.
We run experiments on parallel language specific data sets to identify if the model, e.g. can treat German labeled data as English labeled data and vise versa.
We investigate the opportunity to reach similar individual language model performance with a Multi-Lingual Transfer Learning (MLTL) approach compared to fine-tune on each language in a mono-lingual setup.
For the comparison both models use the same amount of training data, MLTL approach with a mixed language labeled data and language specific for mono-lingual.

In this paper, we investigate the opportunity to reach similar individual language model performance with a Multi-Lingual Transfer Learning (MLTL) approach compared to train each language in a mono-lingual setup.
when fine-tuning on a multi-lingual training set compared to fine-tune each language individually (mono-lingual) with the same amount of data.


We compare three/two?? different approaches/model architectures.
First, we experiment with Multilingual BERT (M-BERT) as a baseline model, re-leased by \cite{mBERT} as a single language model pre-trained on the concatenation of mono-lingual Wikipedia corpora from 104 languages.
Second, we propose a language-adversarial training approach to allow for extracting language invariant features with respect to the language shift.
Model performance is evaluated on an extended ATIS data set \cite{atis} and Alexa in-house data.
We consider bi-lingual and tri-lingual models, considering the need in our Production systems.
???The proposed language-adversarial approach beats all baseline models and also shows lower training times....
\label{introduction}



